Conflict-Free Coloring of Planar Graphs

A conflict-free k-coloring of a graph assigns one of k different colors to some of the vertices such that, for every vertex v, there is a color that is assigned to exactly one vertex among v and v's neighbors. Such colorings have applications in wireless networking, robotics, and geometry, and are well-studied in graph theory. Here we study the natural problem of the conflict-free chromatic number chi_CF(G) (the smallest k for which conflict-free k-colorings exist). We provide results both for closed neighborhoods N[v], for which a vertex v is a member of its neighborhood, and for open neighborhoods N(v), for which vertex v is not a member of its neighborhood. For closed neighborhoods, we prove the conflict-free variant of the famous Hadwiger Conjecture: If an arbitrary graph G does not contain K_{k+1} as a minor, then chi_CF(G) <= k. For planar graphs, we obtain a tight worst-case bound: three colors are sometimes necessary and always sufficient. We also give a complete characterization of the computational complexity of conflict-free coloring. Deciding whether chi_CF(G)<= 1 is NP-complete for planar graphs G, but polynomial for outerplanar graphs. Furthermore, deciding whether chi_CF(G)<= 2 is NP-complete for planar graphs G, but always true for outerplanar graphs. For the bicriteria problem of minimizing the number of colored vertices subject to a given bound k on the number of colors, we give a full algorithmic characterization in terms of complexity and approximation for outerplanar and planar graphs. For open neighborhoods, we show that every planar bipartite graph has a conflict-free coloring with at most four colors; on the other hand, we prove that for k in {1,2,3}, it is NP-complete to decide whether a planar bipartite graph has a conflict-free k-coloring. Moreover, we establish that any general} planar graph has a conflict-free coloring with at most eight colors.

==> 05b-outerplanar-graphs-poly.tex <==
% !TEX root = ./main.tex
\subsubsection{Algorithm for outerplanar graphs.}
In this section, we give a high-level description of the algorithm that computes an optimal conflict-free $k$-coloring of $G$ and the details can be found in the appendix. Let $G = (V,E)$ be an arbitrary outerplanar graph. The neighborhood $N[e]$ of an edge $e=(v,w)$ is defined as $N[v] \cup N[w]$. Consider the dual graph $D = (V_D,E_D)$ of $G$ whose vertices correspond to the faces and whose edges correspond to shared vertices or edges between the faces in $G$. We call the elements of $V_D$ and $E_D$ \emph{nodes} and \emph{links}, respectively, to avoid any confusions with vertices and edges of $G$.  As $G$ is outerplanar, it follows that $D$ is a tree. We choose an arbitrary node $F \in V_D$ as a root of $D$. Thus, each node $v$ has a unique parent node and optionally some attached subtrees that are rooted at the child nodes of $v$.
	
	For each $e \in E_D$, consider one of the subtree, $D_e$, that is obtained by deleting $e$ such that $F \notin D_e$. Let~$G_e \subseteq G$ be the graph that is dual to $D_e$. 
	
	Next, we give a \textit{non-serial dynamic programming} approach, that computes an optimal conflict-free $k$-coloring of $G$. The key idea in our approach are the \textit{configurations} of vertices. Intuitively, a \emph{configuration}, $c_v$, of a vertex $v$ encodes by which colored vertices $v$ is uniquely seen and in which color $v$ is colored, see Definition~\ref{def:edgedonf} for details. The configurations $c_u$ and $c_v$ of the two vertices $u$ and $v$ are combinable if the coloring (of $N[u]$) that is induced by $c_u$ does not \textit{conflict} with the coloring (of $N[v]$) induced by $c_v$ and vice versa, see Definition~\ref{def:combvertexconfig}. A \emph{configuration $c_e$} of an edge $e=(u,v)$ is a pair of configurations $(c_u,c_v)$ for $u$ and $v$ such that $c_u$ and $c_u$ are \emph{combinable}, see Definition~\ref{def:configedges} for details. Thus, for each edge $e \in E$, the number of different configurations is upper-bounded by $\mathcal{O}(n^{2k})$.
	
	Informally spoken, we say that a configuration $c_e$ of an edge $(u,v) = e \in E$ \emph{corresponds} to a partial $k$-coloring if $\chi$ and $c_e$ require the same coloring of vertices from $N[u] \cup N[v]$, see Definition~\ref{def:correspond}.

	\begin{restatable}{lemma}{configuration}
\label{lem:coloringVSconfiguration}
		For each conflict-free $k$-coloring of $G$ there is a set of configurations $\bigcup_{e \in E} c_e$ (and vice versa) such that (1) $\chi$ restricted to $N[e]$ corresponds to $c_e$ and (2) $c_{e_1} = (c_u,c_v)$ and $c_{e_2} = (c_v,c_w)$ for all edges $e_1 = (u,v), e_2=(v,w) \in E$.
	\end{restatable}
	
	For each link~$e=(f_1,f_2) \in E_D$ there is even exactly one shared vertex $v \in f_1 \cap f_2$ or exactly one shared edge $(v,w) \in f_1 \cap f_2$, because $G$ is outerplanar. We call these vertices and edges \emph{bridge vertices} and \emph{bridge edges}. Note that a bridge vertex may also be a vertex of a bridge edge. 
	
	
	
\begin{figure}[h]
\centering
\includegraphics[width=6cm,height=6cm,keepaspectratio]{cf-k-outerplanar_DP}
\caption{Graph construction of faces, bridges, and the corresponding dual (sub)graphs.}
\label{fig:cf-k-outerplanar_DP}
\end{figure}

	Note, on the one side, for each bridge edge there is exactly one corresponding link $e \in E_D$. On the other side, for each bridge vertex, there may by several corresponding links $e_1,\dots,e_l \in E_D$. Thus for a bridge $b$, we consider by $G_b$ the subgraph of $G$ that is defined as the union of all $G_e$ such that $e$ is a link that corresponds to $b$. 

	For a configuration $c_b$ of the bridge $b$, we consider the minimal of number (which we call the \emph{score} of $c_b$) of colored vertices over all partial $k$-colorings $\chi_{c_b}$ of $G_b \cup N[b]$ such that each $v \in G_b$ is uniquely seen and such that $\chi_{c_b}$ restricted to $N[b]$ corresponds to $c_b$. 
	
\begin{lemma}
	For $k \in \{ 1,2 \}$, we can compute the scores $\mathcal{S}(c_b)$ for all configurations $c_b$ of all bridge vertices and bridge edges $b$ in $\mathcal{O}(n^{4k+1})$ time.
\end{lemma}
\begin{proof}
	 We iteratively process one leaf $f$ of $D$ as follows and remove it afterwards: Let $e = (f,f') \in E_D$ be the unique edge that is adjacent to $f$. Suppose there is an bridge edge $b = (u,v)$ between $f$ and $f'$. The case in that $f \cap f'$ is a bridge vertex is similar. Let $f = \langle e_1=(u_1,v_1),\dots,e_{\ell} = (u_{\ell}, v_{\ell}) \rangle$ such that $e_1=b$, $v_{\ell} = u_1$, and $v_i = u_{i+1}$ for $i \in \{ 1,\dots,\ell-1 \}$. Based on the scores of all bridges from $f \setminus \{ e_1 \}$, we can compute $\mathcal{S}(c_b)$ by iteratively computing possible configurations of $e_{i+1}$ based on possible configurations for $e_i$ in $\mathcal{O}(n^{4k})$ time, see Algorithm~\ref{alg:singleconfig} for details. As $D$ has $\mathcal{O}(n)$ faces we obtain a running time of $\mathcal{O}(n^{4k+1})$
\end{proof}

\noindent We are now finally ready to give the proof of Theorem~\ref{thm:DPoptimalconflictfreecoloring}:

%\begin{theorem}\label{thm:DPoptimalconflictfreecoloring}
%	Given an outerplanar graph $G$, we can compute an optimal conflict-free $k$-coloring of $G$ in $\mathcal{O}(n^{4k+1})$ time.
%\end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:DPoptimalconflictfreecoloring}]
	By applying the approach of Lemma~\ref{lem:coloringVSconfiguration} we can compute the scores of all bridges of $F$. Thus a final application of an approach similar to Algorithm~\ref{alg:singleconfig} to $F$ leads to the minimum number of a conflict-free $k$-coloring of $G$. By the above argument it follows that the computed solution is optimal which can be readout by applying backtracking. 
\end{proof}
	 
	
	
	


